Age Recommendation from Texts and Sentences for Children

Children have less text understanding capability than adults. Moreover, this capability differs among the children of different ages. Hence, automatically predicting a recommended age based on texts or sentences would be a great benefit to propose adequate texts to children and to help authors writing in the most appropriate way. This paper presents our recent advances on the age recommendation task. We consider age recommendation as a regression task, and discuss the need for appropriate evaluation metrics, study the use of state-of-the-art machine learning model, namely Transformers, and compare it to different models coming from the literature. Our results are also compared with recommendations made by experts. Further, this paper deals with preliminary explainability of the age prediction model by analyzing various linguistic features. We conduct the experiments on a dataset of 3, 673 French texts (132K sentences, 2.5M words). To recommend age at the text level and sentence level, our best models achieve MAE scores of 0.98 and 1.83 respectively on the test set. Also, compared to the recommendations made by experts, our sentence-level recommendation model gets a similar score to the experts, while the text-level recommendation model outperforms the experts by an MAE score of 1.48.

==> section_6_prediction_experiments.tex <==

\section{Age Prediction Experiments}
\label{sec:age_pred_experiments}
We considers age prediction as a regression task. This section details the different approaches and machine learning models for age prediction from a text/sentence, and shows the experimental results. 

\subsection{Experiment Protocols}
The age prediction approaches studied here are (a) end-to-end text-level (directly prediction from text), (b) sentence-level, and (c) aggregation text-level. In aggregation approach, the sentence-level predictions are aggregated to make a text-level global prediction.
Moreover, in each approach, a text/sentence is transformed into a feature vector of real numbers. This paper studies mainly two kinds of features: (a) embedding features and (b) linguistic expert features.

Finally the feature vectors are fed to a prediction model. Here we study the following regression models.

% \subsection{Regression Models}
\subsubsection{Regression Models}
\paragraph{\normalfont \textbf{CamemBERT} French language model relies on a RoBERTa architecture~\cite{DBLP:journals/corr/abs-1907-11692}, which includes positional encoding and multi-head masking with attention mechanism to learn the language representation. It bidirectionally learns contextual relations from words in all positions unlike the sequential learning in RNN architecture. A pretrained CamemBERT provides also the contextual vector of a word or sentence (mean of the word-vectors in a sentence). CamemBERT offers performing single-output regression task. For age-range prediction, given a sentence as input, two CamemBERT models are employed to predict the lower bound and upper bound separately.
}

\paragraph{\normalfont A \textbf{RNN} model e.g., GRU~\cite{cho2014learning} are able to learn one-way long-term dependencies of a sequence. In a RNN model of age prediction, the input is the sequence of words from the input sentence. Each word goes through a projection layer set with pre-trained word embeddings, before entering the RNN layer. The output of this model is directly two real-values as the lower bound and upper bound of an age-range.}

\paragraph{\normalfont A \textbf{Feed-forward} is a multilayer perceptron network with an input layer, hidden layer(s), and an output layer. In age prediction task, the FF model takes an average vector of word embeddings of size N representing a sequence of words of a sentence, and directly outputs the lower bound and upper bound of an age-range.}

\paragraph{\normalfont A \textbf{Random Forest} is an ensemble learning model to perform classification or regression task which combines multiple decision trees to make the final prediction. A random forest reduces the overfitting and gets rid of the limitations of a decision tree algorithm. It also directly outputs the lower bound and upper bound of an age-range.}

% Each neural network model is run for 3 times to verify the robustness of the model and the average of the predicted ages is reported as the final one. 

\begin{table}[t]
\scriptsize
\begin{center}
	\setlength{\tabcolsep}{2pt}
	\renewcommand{\arraystretch}{2}
	\begin{tabular}{ |l|l|l|}
	 \hline
\textbf{Model} & \textbf{Text Prediction} & \textbf{Sentence Prediction} \\ \hline
\textbf{Feed-forward} & 
\makecell[l]{hidden\_layers = 6, hidden\_units = 200, \\ activation = ReLU, epoch = 500} & \makecell[l]{hidden\_layers = 6, hidden\_units = 200, \\ activation = ReLU, epoch = 500} \\ \hline
\textbf{Random Forest} & \makecell[l]{nb\_estimators = 100, criterion = 'gini', \\ nb\_leaf\_node = $\infty$} & \makecell[l]{nb\_estimators = 100, criterion = 'gini', \\ nb\_leaf\_node = $\infty$}\\ \hline
\textbf{GRU} & \makecell[l]{units = 128,\\ activation = tanh, batch\_size = 128,\\ drop\_out = 0.20, epoch = 50} & Not Used \\ \hline
\textbf{CamemBERT} & Not Used & \makecell[l]{max\_sent.\_len = 100, lr = 1e-5,\\ batch\_size = 32, epoch = 3} \\
\hline
\end{tabular}
\end{center}
\caption{Hyper-parameters used in different models for fine-tuning purpose}
\label{table:hyper_param} 
\end{table}

% \subsection{Training and Parameter Tuning}
\subsubsection{Training and Parameter Tuning}
To feed a model, the tokens of a sentence (or a text) are presented by the word vectors from two embeddings: (i) a CBOW-based word embeddings which is pre-trained on French Wikipedia using fastText~\cite{grave2018learning} with a dimension of $300$, and (ii) CamemBERT contextual embeddings~\cite{martin-etal-2020-camembert} with a dimension of $768$. The sentence/text level vector is derived by taking column-wise mean of the token-vectors. 
However, for the linguistic expert features, primarily each feature (as a real-valued number) is computed at the sentence level, then the text-level feature is derived by taking the mean value of those of all the sentences in a particular text.
The age prediction models are fine-tuned with various hyper-parameters which are detailed in 
Table~\ref{table:hyper_param}.




% \subsection{End-to-end Text-level Models}
\subsection{Age Prediction Scores}
Here we present the scores obtained from the different age prediction models.
\subsubsection{End-to-end text-level predictions}
Although CamemBERT allows regression on long texts (maximum 512 tokens), many texts in our dataset are much larger than this limit. Therefore, in end-to-end age prediction, embedding features are computed from CamemBERT. For a sentence, it gives a vector of $786$ dimensions as a mean-vector of the words in the sentence. A GRU network is trained with the sequence of sentence-vectors. We also train Feed-Forward and Random Forest models with the linguistic Expert features, and combining the Expert features with the GRU predicted min\_age and max\_age. When the predicted ages by a model is used as the features in another model, we call the second one as dependent model. However, an independent model does not depend on any other model.

\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|l||l|l|l|l|}
	 \hline
     & \multicolumn{4}{c|}{\textbf{Validation}} & \multicolumn{4}{c|}{\textbf{Test}}\\
      \hline
	  \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
GRU/(CamemBERT\_sent.\_vector) & 1.42 & 0.30 & 1.97 & \textbf{1.39} & 1.18 & 0.35 & 1.40 & \textbf{0.98} \\
Feed-forward/FastText & 1.70 & 1.10 & 2.61 & 1.96 & 1.72 & 1.01 & 1.79 & 1.52 \\
Feed-forward/Expert & 2.31 & 1.95 & 2.71 & 2.42 & 2.15 & 1.90 & 2.51 & 2.22 \\
Random Forest/FastText & 2.08 & 1.33 & 2.84 & 2.23 & 1.80 & 1.21 & 2.19 & 1.78 \\
Random Forest/Expert & 2.04 & 1.40 & 2.42 & 2.06 & 1.70 & 1.35 & 2.18 & 1.78  \\ \hline
Feed-forward/(GRU\_pred.+Expert)* & 1.72 & 0.79 & 2.26 & 1.72 & 1.42 & 0.85 & 1.70 & 1.34 \\
Random Forest/(GRU\_pred.+Expert)* & 1.33 & 0.23 & 1.95 & \textbf{1.34} & 1.05 & 0.26 & 1.37 & \textbf{0.91} \\
\hline
    \end{tabular}
\end{center}
\caption{End-to-end text-level $\mu{}E$ scores (* indicates dependent model)}
\label{table:End-to-end text level muE} 
\end{table}


\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|l||l|l|l|l|}
	 \hline
     & \multicolumn{4}{c|}{\textbf{$\theta\mbox{-}L_2$}} & \multicolumn{4}{c|}{\textbf{$\beta\mbox{-}IE$}}\\
      \hline
	  \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
GRU/CamemBERT\_sent.\_vector & 2.09 & 1.05 & 2.66 & \textbf{1.96} & 1.17 & 0.39 & 1.47 & \textbf{1.02} \\
Feed-forward/FastText & 2.95 & 1.96 & 3.13 & 2.70 & 1.71 & 1.03 & 1.84 & 1.55 \\
Feed-forward/Expert & 3.58 & 3.29 & 4.21 & 3.75 & 2.16 & 1.95 & 2.63 & 2.28 \\
Random Forest/FastText & 3.04 & 2.21 & 3.70 & 3.06 & 1.80 & 1.25 & 2.23 & 1.81 \\
Random Forest/Expert & 2.90 & 2.40 & 3.73 & 3.07 & 1.70 & 1.37 & 2.25 & 1.81 \\ \hline
Feed-forward/(GRU\_pred.+Expert)* & 2.52 & 1.76 & 3.06 & 2.48 & 1.42 & 0.90 & 1.8 & 1.40 \\
Random Forest/(GRU\_pred.+Expert)* & 1.71 & 0.60 & 2.50 & \textbf{1.66} & 1.04 & 0.28 & 1.43 & \textbf{0.94} \\ \hline
    \end{tabular}
\end{center}
\caption{End-to-end text-level 
$\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ scores on test dataset (* indicates dependent model)}
\label{table:End-to-end text-level proposed metrics} 
\end{table}

Table \ref{table:End-to-end text level muE} shows the $\mu{}E$ scores of different models on the validation and test datasets for end-to-end text-level age prediction. As an independent model, GRU with CamemBERT sentence vectors results the best scores for the three genres Encyclopedia (E), Newspaper (N) and Fiction (F) on both datasets. With the FastText embeddings, the Feed-forward model performs the second best.
However, Random Forest performs better than the Feed-forward model when both are trained with the Expert features. Interestingly, as a dependent model, Random Forest with the combination of GRU predicted min\_age, max\_age, and the Expert features obtains a little better score than the GRU model. Also in terms of the proposed metrics, $\theta\mbox{-}L_2$ and  $\beta\mbox{-}IE$, GRU with CamemBERT sentence vectors outperforms other models as shown in Table \ref{table:End-to-end text-level proposed metrics}. These results indicate that the CamemBERT sentence vector are very effective for age prediction. It is as expected because CamemBERT holds the contextual information of the words in a sentence, and such information helps a NN model to extract useful hidden features.


% \subsection{Sentence-level Models}
\subsubsection{Sentence-level predictions}
For the sentence level experiments, we employ a pretrained CamemBERT as a regression model by fine-tuning it with our training data. CamemBERT does not allow multi-value regression. Therefore,  this paper trains two CamemBERT models separately to predict the lower bound (minimum age) and the upper bound (maximum age) of an age range for sentence level age prediction. Later the mean age is derived from the predicted bounds. However, Feed-forward and Random Forest models are trained to directly predict the age range like the end-to-end age prediction.

\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|l||l|l|l|l|}
	 \hline
     & \multicolumn{4}{c|}{\textbf{Validation}} & \multicolumn{4}{c|}{\textbf{Test}}\\
      \hline
	  \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
CamemBERT/- & 1.93 & 1.3 & 2.21 & \textbf{2.00} & 2.02 & 1.28 & 1.94 & \textbf{1.83}\\
Feed-forward/FastText & 2.31 & 1.65 & 2.86 & 2.53 & 2.41 & 1.61 & 2.38 & 2.24 \\
Feed-forward/Expert & 2.75 & 2.60 & 2.94 & 2.84 & 2.75 & 2.51 & 2.68 & 2.66 \\
Feed-forward/(FastText+Expert) & 2.19 & 1.60 & 2.87 & 2.49 & 2.31 & 1.55 & 2.39 & 2.21 \\
Random Forest/FastText & 2.42 & 2.15 & 2.43 & 2.39  & 2.68 & 2.02 & 2.01 & 2.15 \\
Random Forest/Expert & 2.41 & 2.23 & 2.41 & 2.39 & 2.62 & 2.17 & 2.04 & 2.19 \\ \hline
Feed-forward/(CamemBERT\_pred.+Expert)* & 2.08 & 1.38 & 2.71 & 2.34 & 2.08 & 1.34 & 2.33 & 2.09 \\ 
Random Forest/(CamemBERT\_pred.+Expert)* & 1.97 & 1.22 & 2.42 & \textbf{2.12} & 2.00 & 1.18 & 1.98 & \textbf{1.83} \\
\hline
    \end{tabular}
\end{center}
\caption{Sentence level $\mu{}E$ scores (* indicates dependent model)}
\label{table:Sentence level muE} 
\end{table}


\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|l||l|l|l|l|}
	 \hline
     & \multicolumn{4}{c|}{\textbf{$\theta\mbox{-}L_2$}} & \multicolumn{4}{c|}{\textbf{$\beta\mbox{-}IE$}}\\
      \hline
	  \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
CamemBERT/- & 3.49 & 2.44 & 3.41 & \textbf{3.25} & 2.13 & 1.38 & 2.03 & \textbf{1.93} \\
Feed-forward/FastText & 3.95 & 2.81 & 4.00 & 3.77 & 2.40 & 1.66 & 2.47 & 2.30\\
Feed-forward/Expert & 4.42 & 4.11 & 4.46 & 4.39 & 2.73 & 2.54 & 2.79 & 2.73\\
Feed-forward/(FastText+Expert) & 3.80 & 2.72 & 4.01 & 3.72 & 2.31 & 1.60 & 2.48 & 2.28\\
Random Forest/FastText & 4.29 & 3.47 & 3.48 & 3.65 & 2.66 & 2.08 & 2.09 & 2.20 \\
Random Forest/Expert & 4.22 & 3.67 & 3.56 & 3.72 & 2.62 & 2.21 & 2.14 & 2.25 \\ \hline
Feed-forward/(CamemBERT\_pred.+Expert)* & 3.42 & 2.42 & 3.93 & 3.54 & 2.08 & 1.39 & 2.42 & 2.16 \\
Random Forest/(CamemBERT\_pred.+Expert)* & 3.28 & 2.16 & 3.41 & \textbf{3.15} & 1.99 & 1.25 & 2.05 & \textbf{1.89}\\
 \hline
    \end{tabular}
\end{center}
\caption{Sentence-level 
$\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ scores on test dataset (* indicates dependent model)}
\label{table:Sentence-level proposed metrics} 
\end{table}

Table \ref{table:Sentence level muE} details the sentence level $\mu{}E$ scores on the validation and test datasets for the three genres. The CamemBERT model having no explicit feature achieves the best scores on both datasets for each genre. In contrast, Feed-forward model performs worse than other models with different feature combinations. Interestingly, on Feed-forward, we notice that FastText word embeddings features perform better than the Expert features. The combination of Expert and FastText embeddings features improves a little over the Expert features but seems not significant. Like the end-to-end text-level, Random Forest with Expert features gets better score than the Feed-forward one. 
However, as dependent models, the Feed-forward and Random Forest (with the combination of CamemBERT predicted min-age and max-age with the Expert features) do not improve the scores over the CamemBERT. 

We also observe the $\theta\mbox{-}L_2$ $\beta\mbox{-}IE$ scores (Table \ref{table:Sentence-level proposed metrics}) for the sentence level age prediction on the test dataset and notice the coherency of the performances by different models like with $\mu{}E$ scores.
These scores show that CamemBERT model significantly outperforms the other models without requiring any explicit feature engineering. It is not surprising that the sentence level scores are worse than the end-to-end text-level scores as the training sentences are not annotated by the experts rather it is done based on the text annotations which leads to imperfect sentence annotation.


% \subsection{From Sentences to Text}
\subsubsection{From sentences to text-level predictions}

The sentence level scores still look very decent and it motivates us to explore aggregation of sentence level predictions to make a text-level global prediction. Here we study the mean aggregation which derives the mean value from the predicted ages of the sentences in a text.

\begin{table}[t]
    \scriptsize
\begin{center}
    \setlength{\tabcolsep}{4pt}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{|l|l|l|l|l||l|l|l|l|}
     \hline
     & \multicolumn{4}{c|}{\textbf{Validation}} & \multicolumn{4}{c|}{\textbf{Test}}\\
      \hline
      \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
CamemBERT/- & 1.86 & 1.12 & 1.94 & \textbf{1.72} & 1.92 & 1.16 & 1.73 & \textbf{1.59} \\
Feed-forward/FastText & 2.11 & 1.33 & 2.48 & 2.09 & 2.21 & 1.36 & 1.91 & 1.80 \\ 
Feed-forward/Expert & 2.31 & 2.12 & 2.83 & 2.50 & 2.46 & 2.08 & 2.41 & 2.32 \\ 
Feed-forward/(FastText+Expert) & 2.01 & 1.29 & 2.47 & 2.04 & 2.12 & 1.30 & 1.93 & 1.76 \\
Random Forest/FastText & 2.45 & 2.14 & 2.84 & 2.55 & 2.67 & 2.07 & 2.42 & 2.37 \\
Random Forest/Expert & 2.44 & 2.23 & 2.93 & 2.60 & 2.60 & 2.21 & 2.53 & 2.44 \\ \hline
% Feed-forward/(CamemBERT\_pred.+Expert)* & 1.90 & 1.01 & 2.22 & 1.83 & 1.93 & 1.00 & 1.75 & 1.55 \\ \hline
% Random Forest/(CamemBERT\_pred.+Expert)* & 1.93 & 1.02 & 2.2 & 1.83 & 1.96 & 1.03 & 1.75 & 1.56 \\
    \end{tabular}
\end{center}
\caption{Text level $\mu{}E$ scores by Mean-aggregation %(* indicates dependent model)
}
\label{table:Text level muE by Mean-Aggregation} 
\end{table}


\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|l||l|l|l|l|}
	 \hline
     & \multicolumn{4}{c|}{\textbf{$\theta\mbox{-}L_2$}} & \multicolumn{4}{c|}{\textbf{$\beta\mbox{-}IE$}}\\
      \hline
	  \textbf{Model/Features} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} & \textbf{E} & \textbf{N} & \textbf{F} & \textbf{Overall} \\ \hline
CamemBERT/- & 3.27 & 2.18 & 3.07 & \textbf{2.83} & 1.97 & 1.21 & 1.78 & \textbf{1.64}\\
Feed-forward/FastText & 3.61 & 2.42 & 3.35 & 3.10 & 2.19 & 1.37 & 1.96 & 1.82\\
Feed-forward/Expert & 3.97 & 3.48 & 4.08 & 3.86 & 2.42 & 2.06 & 2.49 & 2.34\\
Feed-forward/(FastText+Expert) & 3.49 & 2.33 & 3.37 & 3.05 & 2.10 & 1.31 & 1.98 & 1.78\\
Random Forest/FastText & 4.26 & 3.46 & 4.08 & 3.92 & 2.63 & 2.04 & 2.48 & 2.38 \\
Random Forest/Expert & 4.17 & 3.65 & 4.28 & 4.05 & 2.56 & 2.18 & 2.63 & 2.46\\ 
% \hline
% Feed-forward/(CamemBERT\_pred.+Expert)* & 3.21 & 1.89 & 3.14 & \textbf{2.73} & 1.91 & 1.03 & 1.82 & \textbf{1.58}\\
% Random Forest/(CamemBERT\_pred.+Expert)* & 3.25 & 1.93 & 3.14 & 2.76 & 1.93 & 1.06 & 1.81 & 1.59\\

 \hline
    \end{tabular}
\end{center}
\caption{Text level 
$\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ scores by mean-aggregation on test dataset 
%(* indicates dependent model)
}
\label{table:mean-aggregation proposed metrics} 
\end{table}

As shown in Table ~\ref{table:Text level muE by Mean-Aggregation}, the mean-aggregation gives very good $\mu{}E$ scores to predict age for a text especially for the CamemBERT model. CamemBERT obtains $\mu{}E$ scores of $1.72$ and $1.59$ on the validation and test datasets which are $0.33$ and $0.61$ points worse than the best (GRU with CamemBERT sentence vectors) end-to-end model. Although, Feed-forward performs better than Random Forest, both get some good scores on the validation and test datasets. Like the sentence-level and end-to-end text-level, here again we notice that with the Feed-forward model, the FastText embeddings performs better than the Expert features. The combination of FastText and Expert features gets insignificantly a little better score over FastText only. 
Similar behaviour is noticed with the $\theta\mbox{-}L_2$ $\beta\mbox{-}IE$ scores on the test dataset as shown in Table~\ref{table:mean-aggregation proposed metrics}.  

Overall, the scores by mean-aggregation are very promising and this aggregation method provides significant insights on the age-prediction particularly for the authors view-point. This approach can be very effective for an author to incrementally verify a text for a target age.

% \subsection{Comparison of Predictions per Age and Age-range}
\subsubsection{Comparison of predictions per age and age-range}
Up to now, GRU/CamemBERT and Feed-forward/FastText are the best performing two models for the end-to-end and sentence level age prediction. Here we compare their prediction performances for each age and age-range.

\begin{figure}[t]%[ht]
    \centering
    \includegraphics[width=\linewidth]{lre_texttokids_age_recommendation/figures/score_charts.png}
\caption{Per age (a and b), and per age-range (c and d) $\mu{}E$ scores at the text level (a and c) and sentence level (b and d) on test set}
\label{fig:score_charts}
\end{figure}

Fig.~\ref{fig:score_charts} shows the $\mu{}E$ scores per age (a and b), and per age-range (c and d) at the text level (a and c) and sentence level (b and d) on test set. Almost in all cases (except text level scores per age-range), the GRU/CamemBERT-vector (text level) and CamemBERT (sentence level) outperform the Feed-forward/FastText model.

For end-to-end text level age prediction, GRU/CamemBERT-vector performs better for predicting ages of 8 to 12 years (older children) and 14 to 18 years (adults). For other ages, the two models perform quite similar. However, in sentence level age prediction, CamemBERT gets much better scores for child-ages than adult-ages. 
Overall, CamemBERT has outstanding contributions in age prediction task.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Comparison with Experts}
\label{sec:experts}
This section compares the predictions from our best models with those of three psycho-linguist experts on sentences and texts. To do so, the experts were requested to annotate $20$ texts from the test set and $80$ sentences randomly selected from these $20$ texts. The different models are applied on the same sentences and texts. Table~\ref{table:expert_test_scores} compares $\mu{}E$, $\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ scores measured for the CamemBERT models, every expert, and when averaging the expert's predictions. 

\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{3pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{ |l|l|l|l||l|l|l|l|}
	 \hline
\multicolumn{4}{|c|}{\textbf{Sentence Prediction}} & \multicolumn{4}{c|}{\textbf{Text Prediction}}\\ \hline
\textbf{Model} & \textbf{$\mu{}E$} & \textbf{$\theta\mbox{-}L_2$} & \textbf{$\beta\mbox{-}IE$} & \textbf{Model}  & \textbf{$\mu{}E$} & \textbf{$\theta\mbox{-}L_2$} & \textbf{$\beta\mbox{-}IE$} \\
\hline
% Naive & 5.36 & 8.22 & 4.94 &  \multicolumn{1}{c|}{--} & 4.55 & 7.07 & 4.23 \\
% \hline
\multirow{2}{*}{CamemBERT} & \multirow{2}{*}{3.43} &  \multirow{2}{*}{5.54} & \multirow{2}{*}{3.21} & Mean Aggr. (CamemBERT) & 2.95 & 4.83 & 2.76 \\
 & & & & End-to-end (GRU/CamemBERT\_vector) & \textbf{1.47} & 2.72 & 1.43 \\
\hline %\hline
Expert 1 & 3.28 & 5.23 & 3.27 & \multicolumn{1}{l|}{Expert 1} & 2.60 & 4.23 & 2.60 \\ 
Expert 2 & 3.25 & 5.28 & 3.33 & \multicolumn{1}{l|}{Expert 2} & 3.50 & 5.76 & 3.63 \\
Expert 3 & 3.18 & 5.28 & 3.26 & \multicolumn{1}{l|}{Expert 3} & 2.72 & 4.47 & 2.70 \\
\hline
Expert mean & 2.90 & 4.76 & 2.93 & \multicolumn{1}{l|}{Expert mean} & 2.95 & 4.81 & 2.95 \\
\hline
    \end{tabular}
\end{center}
\caption{Text level $\mu{}E$, $\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ for the expert annotated 80 sentences and 24 texts from the test set.}
\label{table:expert_test_scores} 
\end{table}



\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{3pt}
	\renewcommand{\arraystretch}{1.9}
	\begin{tabular}{|l|l|l|l|l|l|}
	 \hline
	  \textbf{Sentence} & \makecell[c]{\textbf{Actual Age} \\ \textbf{Range / Mean}} & \makecell[c]{\textbf{CamemBERT}\\ \textbf{Range / Mean}} & \textbf{$\mu{}E$} & \textbf{$\theta\mbox{-}L_2$} & \textbf{$\beta\mbox{-}IE$} \\ 
	  \hline

\makecell[l]{\textbf{1.} And the fox, which open ears\\everywhere hears a day.} & [4, 6] / 5.0 & \textbf{[3.65, 7.20] / 5.43} & 0.43 & 2.19 & 1.02 \\ 
\hdashline
\makecell[l]{\textbf{2.} This afternoon, Tremolo was to\\ play at a funeral.} & [8, 11] / 9.5  & \textbf{[8.98, 11.27] / 10.13} & 0.62 & 1.27 & 0.60 \\
\hdashline
\makecell[l]{\textbf{3.} If we wait later, it is more complicated.} & [12, 14] / 13.0 & [7.80, 12.04] / 9.92 & 3.08 & 5.30 & 3.62 \\
\hdashline
\makecell[l]{\textbf{4.} By then, you will have had time\\ to comfort a little girl who has already\\ shed tears on her fault.} & [14, 18] / 16.0 &  [7.35, 11.50] / 9.43 & 6.57 & 9.80 & 6.60 \\
      \hline
    \end{tabular}
\end{center} % B-IE corrected
\caption{Examples of age prediction by the CamemBERT model for some expert-annotated sentences. Here the sentences are translated in English while the French version available in the Appendix)}
\label{table:example_preds} 
\end{table}

The CamemBERT model gets high $\mu{}E$, $\theta\mbox{-}L_2$ and $\beta\mbox{-}IE$ scores at the sentence level but still performs quite similar to the individual experts. The CamemBERT model gets worse scores than the expert-mean. At the text level, CamemBERT with mean-aggregation obtains the same $\mu{}E$ as that of the expert-mean. As an end-to-end model, GRU/CamemBERT\_vector significantly outperforms the experts. These results indicate that our proposed models perform better than human annotators. 
Table~\ref{table:example_preds} presents some sentence level predictions where the sentences are annotated by experts. The proposed CamemBERT model gives very good prediction for the first two sentences while it fails very badly for the last two.



% text lenghts in tokens:min=20, max=27015, mean=690, median=715, Q1=417, Q2=715, Q3=961

% 500 +: 2438 / 3697 :: 65.95 %
% 600 +: 2100 / 3697 :: 56.80 %
% 700 +: 1871 / 3697 :: 50.61 %
% 800 +: 1642 / 3697 :: 44.41 %
% 900 +: 1259 / 3697 :: 34.05 %
% 1000 +: 701 / 3697 :: 18.96 %
% 1100 +: 237 / 3697 :: 6.41 %
% 1200 +: 131 / 3697 :: 3.54 %
% 1300 +: 91 / 3697 :: 2.46 %
% 1400 +: 76 / 3697 :: 2.06 %
% 1500 +: 63 / 3697 :: 1.70 %


% Naive-scores
% Encyclop	Newspaper	Fiction
% Expert::dev::sentence-level-mae-mean
% 2.67	2.61	2.94	2.82
% Expert::test::sentence-level-mae-min-max-mean
% 3.26	2.63	2.2	2.5
% Expert::dev::sentence-level-MED_ANGLE_ALPHA
% 4.3	4.25	4.78	4.57
% Expert::test::sentence-level-MED_ANGLE_ALPHA
% 5.11	4.28	3.83	4.18
% Expert::dev::sentence-level-ASYM_IE_BETA
% 2.65	2.56	3.06	2.87
% Expert::test::sentence-level-ASYM_IE_BETA
% 3.22	2.59	2.35	2.58

% Expert::dev::text-level-mae-mean
% 2.8	2.94	3.78	3.25
% Expert::test::text-level-mae-mean
% 3.24	2.94	3.12	3.1
% Expert::dev::text-level-MED_ANGLE_ALPHA
% 4.44	4.69	5.97	5.15
% Expert::test::text-level-MED_ANGLE_ALPHA
% 5.07	4.69	5.13	4.98
% Expert::dev::text-level-ASYM_IE_BETA
% 2.76	2.9	3.93	3.29
% Expert::test::text-level-ASYM_IE_BETA
% 3.21	2.9	3.31	3.16

==> section_7_feature_analysis_EN.tex <==
\section{Feature Analysis}
\label{sec:feature_analysis}
% data stat: 
% about the features
% scores per age

Overall the age recommendation models obtain very decent scores. Although the \textit{Expert} feature set alone does not achieve the best score, it allows us to analyse which linguistic properties have higher contributions for age recommendation. This section explores feature selection by different approaches.

\subsection{Correlation Between Feature and Age}
At this point, we are interested to measure the correlation between the features and age (on test set) to identify the most contributory features. First correlation is measured between each expert-feature and the real ages at the sentence and text levels, and then done similar with the recommended ages for two models, [GRU/T\textsubscript{CB}, Feed-forward/GRU\_pred.$\oplus$T\textsubscript{Expert}] (for text level recommendation) and [CamemBERT/-, Feed-forward/CamemBERT\_pred.$\oplus$S\textsubscript{Expert}] (for sentence level recommendation). We hypothesize that the top ranked correlated features will be similar for the real age and recommended age for a good age recommendation model. This section refers Pearson correlation coefficient as the correlation score.

\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l||l|l|l|l|l|}
	 \hline
     & \multicolumn{3}{c||}{\textbf{Real Age}} & \multicolumn{5}{c|}{\textbf{Recommended Age}}\\
      \hline
      & \multicolumn{3}{c||}{} & \multicolumn{2}{c|}{\textbf{GRU or CamemBERT}} & \multicolumn{2}{c|}{\makecell{\textbf{Expert} $\oplus$\\ \textbf{[GRU or CamemBERT]}}} & \\
      \hline
	  \textbf{Features} & \textbf{Text} & \textbf{Senence} & \textbf{Avg.*} & \textbf{Text} & \textbf{Sentence} & \textbf{Text} & \textbf{Sentence} & \textbf{Avg.} \\ \hline
PhonemeNumberAvg & 0.56 / 2 & 0.25 / 1 & 0.40 / 1 & 0.48 / 3 & 0.27 / 1 & 0.53 / 3 & 0.23 / 1 & 0.38 / 2 \\
PhonemeNumberStd & 0.58 / 1 & 0.22 / 2 & 0.40 / 2 & 0.52 / 1 & 0.26 / 2 & 0.56 / 1 & 0.20 / 5 & 0.38 / 1 \\
WordLengthStd & 0.54 / 3 & 0.19 / 7 & 0.37 / 3 & 0.50 / 2 & 0.25 / 4 & 0.53 / 2 & 0.20 / 8 & 0.37 / 3 \\
LemmaDiversity & 0.50 / 4 & 0.22 / 4 & 0.36 / 4 & 0.48 / 6 & 0.24 / 5 & 0.49 / 5 & 0.21 / 3 & 0.35 / 5 \\
SentenceLength & 0.49 / 5 & 0.22 / 3 & 0.36 / 5 & 0.48 / 4 & 0.25 / 3 & 0.49 / 6 & 0.21 / 2 & 0.36 / 4 \\
WordLengthAvg & 0.49 / 6 & 0.20 / 5 & 0.35 / 6 & 0.43 / 8 & 0.23 / 6 & 0.47 / 7 & 0.20 / 6 & 0.33 / 7 \\
SymbolProportion & 0.49 / 7 & 0.20 / 6 & 0.35 / 7 & 0.43 / 9 & 0.23 / 7 & 0.47 / 8 & 0.20 / 7 & 0.33 / 8 \\
DependencyTreeDepth & 0.48 / 8 & 0.19 / 8 & 0.34 / 8 & 0.48 / 5 & 0.22 / 8 & 0.50 / 4 & 0.20 / 4 & 0.35 / 6 \\
DependencyMaxDistance & 0.47 / 9 & 0.18 / 9 & 0.32 / 9 & 0.44 / 7 & 0.20 / 9 & 0.46 / 9 & 0.18 / 9 & 0.32 / 9 \\
GraphemeConfusionStd & 0.47 / 10 & 0.16 / 10 & 0.31 / 10 & 0.41 / 10 & 0.20 / 10 & 0.45 / 10 & 0.16 / 10 & 0.30 / 10 \\
% GraphemeConfusionAvg & 0.40 / 11 & 0.15 / 11 & 0.27 / 11 & 0.32 / 14 & 0.17 / 11 & 0.35 / 13 & 0.14 / 11 & 0.25 / 11 \\
% PointDistMoy & 0.39 / 12 & 0.12 / 12 & 0.26 / 12 & 0.34 / 12 & 0.13 / 13 & 0.38 / 11 & 0.13 / 12 & 0.24 / 13 \\
% PointDistVar & 0.38 / 13 & 0.10 / 14 & 0.24 / 13 & 0.37 / 11 & 0.13 / 12 & 0.37 / 12 & 0.11 / 13 & 0.25 / 12 \\
% depDistMoy & 0.36 / 14 & 0.12 / 13 & 0.24 / 14 & 0.33 / 13 & 0.12 / 14 & 0.35 / 14 & 0.11 / 14 & 0.23 / 14 \\
% NumberOfDependenciesAvg & 0.28 / 15 & 0.09 / 15 & 0.19 / 15 & 0.23 / 15 & 0.07 / 17 & 0.26 / 15 & 0.10 / 16 & 0.17 / 15 \\
\hline
\hline
PhonemeNumberSentence & -0.34 / 2 & -0.15 / 1 & -0.25 / 1 & -0.31 / 3 & -0.16 / 1 & -0.34 / 3 & -0.14 / 1 & -0.24 / 2 \\
PhonemeDiversitySentence & -0.34 / 3 & -0.15 / 2 & -0.25 / 2 & -0.31 / 4 & -0.16 / 2 & -0.34 / 4 & -0.14 / 2 & -0.24 / 3 \\
PhonemeProbStd & -0.37 / 1 & -0.10 / 4 & -0.24 / 3 & -0.39 / 1 & -0.15 / 3 & -0.43 / 1 & -0.12 / 4 & -0.27 / 1 \\
PhonemesDiversityStd & -0.32 / 6 & -0.14 / 3 & -0.23 / 4 & -0.25 / 6 & -0.15 / 4 & -0.30 / 6 & -0.14 / 3 & -0.21 / 4 \\
StopWordsProportion & -0.33 / 5 & -0.08 / 5 & -0.20 / 5 & -0.31 / 5 & -0.09 / 6 & -0.32 / 5 & -0.05 / 6 & -0.19 / 5 \\
TemporalConnectorProportion & -0.34 / 4 & -0.04 / 10 & -0.19 / 6 & -0.32 / 2 & -0.04 / 10 & -0.35 / 2 & -0.04 / 9 & -0.19 / 6 \\
LoveProportion & -0.29 / 8 & -0.06 / 7 & -0.17 / 7 & -0.23 / 7 & -0.07 / 7 & -0.27 / 7 & -0.05 / 7 & -0.15 / 7 \\
JoyProportion & -0.29 / 7 & -0.05 / 8 & -0.17 / 8 & -0.17 / 10 & -0.06 / 8 & -0.22 / 9 & -0.04 / 8 & -0.12 / 10 \\
GraphemeProbStd & -0.21 / 10 & -0.08 / 6 & -0.14 / 9 & -0.16 / 11 & -0.11 / 5 & -0.22 / 10 & -0.10 / 5 & -0.14 / 8 \\
PropOpposition & -0.24 / 9 & -0.04 / 9 & -0.14 / 10 & -0.23 / 8 & -0.05 / 9 & -0.23 / 8 & -0.04 / 10 & -0.14 / 9 \\
% BehaviouralTerms & -0.18 / 11 & -0.03 / 12 & -0.10 / 11 & -0.19 / 9 & -0.04 / 11 & -0.20 / 11 & -0.03 / 12 & -0.11 / 11 \\
% peur & -0.16 / 12 & -0.04 / 11 & -0.10 / 12 & -0.14 / 12 & -0.02 / 13 & -0.16 / 12 & -0.02 / 13 & -0.09 / 12 \\
% TemporalAdvProportion & -0.12 / 13 & -0.02 / 14 & -0.07 / 13 & 0.00 / 25 & -0.02 / 14 & -0.13 / 13 & -0.03 / 11 & -0.05 / 16 \\
% PropAddition & -0.11 / 14 & -0.02 / 17 & -0.06 / 14 & 0.01 / 26 & -0.02 / 16 & -0.10 / 16 & -0.01 / 20 & -0.03 / 18 \\
% EnumerationConnectorProportion & -0.08 / 16 & -0.02 / 13 & -0.05 / 15 & 0.11 / 24 & -0.01 / 22 & -0.07 / 18 & -0.01 / 19 & 0.00 / 28 \\
    \hline
    \end{tabular}
\end{center}
\caption{Correlation (correlation score / feature rank) of \textit{Expert} features to the real and recommended mean-ages at the text and sentence levels}
\label{table:correlation} 
\end{table}

Table~\ref{table:correlation} shows the top 10 positively correlated (upper part) and top 10 negatively correlated (bottom part) features with different settings. Each correlation score is presented with its rank among the features. For example, in second column (Real Age/Text), the correlation score for \textit{PhonemeNumberStd} (0.58 / 1) is 0.58 with the rank of 1. From this table, it is very clear that the top 10 positively correlated features are common in all settings although their ranks displace a little. Similar characteristics is observed for the top 10 negatively correlated features as well. From the correlation based feature ranking, one can notice that the most important features include \textit{Phonetics}, \textit{SentenceLength} and \textit{DependencyMaxDistance}. 

\subsection{Permutation Feature Ranking}
The idea of permutation feature ranking is to randomly shuffle an individual feature value to break the relationship between the feature and the target value. Thus it measures the drop of performance due to discarding the feature, and finally ranks the features. Here we do it on the test set by employing Random Forest regressor, a built-in library in scikit-learn. First, feature ranking is performed with the expert features (T\textsubscript{Expert} and S\textsubscript{Expert}) at the sentence and text levels, and then combining them with the GRU\_pred. ages (text level) and CamemBERT\_pred. ages (sentence level) as additional features.

\begin{table}[t]
    \tiny
\begin{center}
	\setlength{\tabcolsep}{2pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l||l|l|}
	 \hline
% 	 \textbf{S\textsubscript{Expert} (sentence level)} & \textbf{T\textsubscript{Expert} (text level)} & \textbf{S\textsubscript{Expert}$\oplus$CamemBERT\_pred.} & \textbf{T\textsubscript{Expert}$\oplus$GRU\_pred.}\\
     \multicolumn{2}{|c||}{\textbf{Expert Features}} & \multicolumn{2}{c|}{\textbf{Expert $\oplus$ [CamemBERT\_pred. or GRU pred.] Features}}\\
      \hline
	  \textbf{Sentence level} & \textbf{Text level} & \textbf{Sentence level} & \textbf{Text level} \\ \hline
% 	  PhonemeNumberAvg & PhonemeNumberAvg & CamemBertPredMaxAge & GruPredMinAge \\
% PhonemeNumberStd & SentenceLength & CamemBertPredMinAge & GruPredMaxAge \\
% SentenceLength & PhonemeNumberStd & SadnessProportion & PhonemeProbSentence \\
% PhonemeProbStd & PhonemeProbStd & SurpriseProportion & WordProbAvg \\
% StopWordsProportion & PolarityScore & EnumerationConnectorProportion & WordLengthAvg \\
% NumberOfDependenciesAvg & PhonemeProbSentence & BehaviouralTerms & GraphemeProbAvg \\
% DependencyMaxDistance & DependencyMaxDistance & ContemptProportion & NumberOfDependenciesAvg \\
% WordProbAvg & StopWordsProportion & ConclusionConnectorProportion & NeutralProportion \\
% PhonemesDiversityAvg & WordProbAvg & TemporalAdvProportion & SymbolProportion \\
% PhonemesDiversityStd & GraphemeConfusionAvg & PrideProportion & DependencyTreeDepth \\


PhonemeNumberAvg (0.1021) & PhonemeNumberAvg (0.1596) & CamemBertPredMaxAge (0.2400) & GruPredMinAge (0.4634) \\
PhonemeNumberStd (0.0383) & SentenceLength (0.1425) & CamemBertPredMinAge (0.2099) & GruPredMaxAge (0.4017) \\
SentenceLength (0.0368) & PhonemeNumberStd (0.0847) & SadnessProportion (0.0003) & PhonemeProbSentence (0.0041) \\
PhonemeProbStd (0.0132) & PhonemeProbStd (0.0245) & SurpriseProportion (0.0002) & WordProbAvg (0.0030) \\
StopWordsProportion (0.0130) & PolarityScore (0.0213) & EnumerationConnectorProportion (0.0002) & WordLengthAvg (0.0024) \\
NumberOfDependenciesAvg (0.0110) & PhonemeProbSentence (0.0180) & BehaviouralTerms (0.0001) & GraphemeProbAvg (0.0023) \\
DependencyMaxDistance (0.0086) & DependencyMaxDistance (0.0164) & ContemptProportion (0.0001) & NumberOfDependenciesAvg (0.0019) \\
WordProbAvg (0.0076) & StopWordsProportion (0.0151) & ConclusionConnectorProportion (0.0001) & NeutralProportion (0.0013) \\
PhonemesDiversityAvg (0.0069) & WordProbAvg (0.0143) & TemporalAdvProportion (0.0001) & SymbolProportion (0.0010) \\
PhonemesDiversityStd (0.0063) & GraphemeConfusionAvg (0.0142) & PrideProportion (0.0001) & DependencyTreeDepth (0.0008) \\

% VarFreqOccurence & GraphemeProbAvg & TemporalConnectorProportion & PropCause \\
% PhonemeDiversitySentence & LemmaDiversity & empathie & FrequencePhonemesMoyenne \\
% PhonemeNumberSentence & GraphemeConfusionStd & fierte & PhonemesDiversityAvg \\
% GraphemeProbAvg & DependencyTreeDepth & PropCause & VarFreqOccurence \\
% PhonemeProbSentence & PropConsequence & apaisement & depDistMoy \\
      \hline
    \end{tabular}
\end{center}
\caption{Top 10 \textit{Expert} features (with rank-scores) by permutation feature ranking at the sentence and text levels}
\label{table:permutation feature ranks} 
\end{table}

Table~\ref{table:permutation feature ranks} enlists the top 10 features for different feature combinations at the sentence and text levels. For ranking on the \textit{Expert} features, most of the top ranked features are related to \textit{Phonetics}. Moreover, the \textit{SentenceLength}, \textit{DependencyMaxDistance} and \textit{StopWordsProportion} are found very important features for age recommendation at the sentence and text levels. These features are also seen in the list of top 10 features by correlation based feature ranking in Table~\ref{table:correlation}.

However, when the ranking is done by Expert$\oplus$[CamemBERT\_pred. or GRU pred.] features, CamemBERT or GRU recommended ages are ranked as the most contributory features at sentence and text levels. Interestingly, the rest of the important features differ significantly between the sentence and text levels. Moreover, for Expert$\oplus$[CamemBERT\_pred. or GRU pred.] setting, the top-ranked \textit{Expert} features do not include the \textit{Phonetics}, \textit{SentenceLength} and \textit{DependencyMaxDistance} features. The reason may be that CamemBERT has already considered these information in its training phase.


\subsection{Ablation Test}
Finally we do an ablation test with different categories of the \textit{Expert} features on the test set. The idea of ablation test is like the permutation feature ranking where an individual feature is shuffled and its impact on the performance is measured. Here ablation test is done with the Feed-forward model,
but instead of shuffling a single feature, all the features of same category are discarded.

% \begin{table}[t]
%     %\small
% \begin{center}
% 	\setlength{\tabcolsep}{2pt}
% 	\renewcommand{\arraystretch}{1.3}
% 	\begin{tabular}{|l|l|l||l|l|}
% 	 \hline
%      & \multicolumn{2}{c|}{\textbf{Sentence Level}} & \multicolumn{2}{c|}{\textbf{End-to-end Text Level}}\\
%       \hline
% 	  \textbf{Features} & \textbf{MAE} & \textbf{MBE} & \textbf{MAE} & \textbf{MBE} \\ \hline
% Expert & 2.68 & 1.42 & 2.13 & 0.84 \\ \hdashline
% Expert-Dependencies & 2.71 & 1.44 & 2.27 & 0.94 \\
% Expert-Person/Number & 2.68 & 1.42 & 2.16 & 0.86 \\
% Expert-Graphemes & 2.65 & 1.39 & 2.18 & 0.87 \\
% Expert-Lexicon & 2.69 & 1.42 & 2.29 & 0.95 \\
% Expert-VerbalTenses& 2.66 & 1.40 & 2.19 & 0.88 \\
% Expert-Phonetics & 2.77 & 1.49 & 2.33 & 0.97 \\
% Expert-Morphosyntax & 2.71 & 1.45 & 2.26 & 0.94 \\
% Expert-Connectors& 2.67 & 1.42 & 2.21 & 0.93 \\
% Expert-Sentiments & 2.69 & 1.43 & 2.18 & 0.85 \\ \hline
%     \end{tabular}
% \end{center}
% \caption{Ablation test MAE (mean-age) and MBE}
% \label{table:Ablation test MAE and MBE} 
% \end{table}


\begin{table}[t]
    %\small
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|}
	 \hline
	  \textbf{Features} & \textbf{Sentence} & \textbf{Text} \\ \hline
\textbf{Expert} & \textbf{2.66} & \textbf{2.22} \\ \hline
Expert - Phonetics & 2.77 / +0.11 & 2.33 / +0.11 \\
Expert - Dependencies & 2.71 / +0.05 & 2.27 / +0.05 \\
Expert - Morphosyntax & 2.71 / +0.05 & 2.26 / +0.04 \\
Expert - Lexicon & 2.69 / +0.03 & 2.29 / +0.07 \\
\hdashline
Expert - Sentiments & 2.69 / +0.03 & 2.18 / -0.04 \\
Expert - Person/Number & 2.68 / +0.02 & 2.16 / -0.06 \\
Expert - Connectors & 2.67 / +0.01 & 2.21 / -0.01 \\
Expert - VerbalTenses & 2.66 / +0.00 & 2.19 / -0.03 \\
Expert - Graphemes & 2.65 / -0.01 & 2.18 / -0.04 \\
\hline
    \end{tabular}
\end{center}
\caption{Ablation test ($\mu{}E$ / $\Delta$) of the \textit{Expert} features with Feed-forward model at the sentence and text levels}
\label{table:Ablation test muE} 
\end{table}

Table~\ref{table:Ablation test muE} presents the $\mu{}E$ scores of the ablation test where almost all the feature categories except \textit{VerbalTenses} and \textit{Grapheme} show positive impacts at sentence level. Interestingly, the \textit{Phonetics, Dependencies, Morphosyntax} and \textit{Lexicon} features have positive impacts at both sentence and text levels. All the feature ranking approaches studied in this paper find the phonetics and dependency features the most common and contributory in any settings. Although these feature categories individually do not have very high impact, they altogether perform quite well in age recommendation task.

==> section_7_feature_analysis_EN_v2.tex <==
\section{Feature Analysis}
\label{sec:feature_analysis}

Overall the age recommendation models obtain very decent scores. Although the \textit{Expert} feature set (with any regressor) does not achieve the best score, it allows us to analyse which linguistic properties have higher contributions in age recommendation. This section explores feature ranking by different approaches.


\subsection{Correlation Between Feature and Age}
At this point, we are interested to measure the correlation (Pearson correlation coefficient) between the features and ages (on test set) to identify the most contributory features. 

\begin{figure}[bt]%[ht]
\centering
\includegraphics[width=0.60\linewidth]{figures/correlation2.png}
\caption{Correlation between expert feature and real age, and expert feature and predicted age}
\label{fig:correlation}
\vspace{-2mm}
\end{figure}


\begin{table}[t]
    \tiny
\begin{center}
	\setlength{\tabcolsep}{2pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l||l|l|l|}
	 \hline
     & \multicolumn{3}{c||}{\textbf{Real Age}} & \multicolumn{3}{c|}{\textbf{Predicted Age}}\\
    %   \hline
    %   & \multicolumn{3}{c||}{} & \multicolumn{3}{c|}{\textbf{GRU or CamemBERT}} \\
      \hline
	  \textbf{Features} & \textbf{Text} & \textbf{Sentence} & \textbf{Avg.*} & \makecell[c]{\textbf{Text} \\ \textbf{(GRU/T\textsubscript{CB})}} & \makecell[c]{\textbf{Sentence} \\ \textbf{(CamemBERT/-)}} & \textbf{Avg.} \\ \hline
PhonemeNumberAvg & 0.56 / 2 & 0.25 / 1 & 0.40 / 1 & 0.48 / 3 & 0.27 / 1 & 0.38 / 2 \\
PhonemeNumberStd & 0.58 / 1 & 0.22 / 2 & 0.40 / 2 & 0.52 / 1 & 0.26 / 2 & 0.39 / 1 \\
WordLengthStd & 0.54 / 3 & 0.19 / 7 & 0.37 / 3 & 0.50 / 2 & 0.25 / 4 & 0.38 / 3 \\
LemmaDiversity & 0.50 / 4 & 0.22 / 4 & 0.36 / 4 & 0.48 / 6 & 0.24 / 5 & 0.36 / 5 \\
SentenceLength & 0.49 / 5 & 0.22 / 3 & 0.36 / 5 & 0.48 / 4 & 0.25 / 3 & 0.37 / 4 \\
WordLengthAvg & 0.49 / 6 & 0.20 / 5 & 0.35 / 6 & 0.43 / 8 & 0.23 / 6 & 0.33 / 7 \\
SymbolProportion & 0.49 / 7 & 0.20 / 6 & 0.35 / 7 & 0.43 / 9 & 0.23 / 7 & 0.33 / 8 \\
DependencyTreeDepth & 0.48 / 8 & 0.19 / 8 & 0.34 / 8 & 0.48 / 5 & 0.22 / 8 & 0.35 / 6 \\
DependencyMaxDistance & 0.47 / 9 & 0.18 / 9 & 0.32 / 9 & 0.44 / 7 & 0.20 / 9 & 0.32 / 9 \\
GraphemeConfusionStd & 0.47 / 10 & 0.16 / 10 & 0.31 / 10 & 0.41 / 10 & 0.20 / 10 & 0.31 / 10 \\
\hline
\hline
PhonemeNumberSentence  &  -0.34 / 2  &  -0.15 / 1  &  -0.25 / 1  &  -0.31 / 3  &  -0.16 / 1  & -0.24 / 2 \\
PhonemeDiversitySentence  &  -0.34 / 3  &  -0.15 / 2  &  -0.25 / 2  &  -0.31 / 4  &  -0.16 / 2  & -0.24 / 3 \\
PhonemeProbStd  &  -0.37 / 1  &  -0.10 / 4  &  -0.24 / 3  &  -0.39 / 1  &  -0.15 / 3  & -0.27 / 1 \\
PhonemesDiversityStd  &  -0.32 / 6  &  -0.14 / 3  &  -0.23 / 4  &  -0.25 / 6  &  -0.15 / 4  & -0.20 / 4 \\
StopWordsProportion  &  -0.33 / 5  &  -0.08 / 5  &  -0.20 / 5  &  -0.31 / 5  &  -0.09 / 6  & -0.20 / 5 \\
TemporalConnectorProp.  &  -0.34 / 4  &  -0.04 / 10  &  -0.19 / 6  &  -0.32 / 2  &  -0.04 / 10  & -0.18 / 6 \\
LoveProportion  &  -0.29 / 8  &  -0.06 / 7  &  -0.17 / 7  &  -0.23 / 7  &  -0.07 / 7  & -0.15 / 7 \\
JoyProportion  &  -0.29 / 7  &  -0.05 / 8  &  -0.17 / 8  &  -0.17 / 10  &  -0.06 / 8  & -0.12 / 10 \\
GraphemeProbStd  &  -0.21 / 10  &  -0.08 / 6  &  -0.14 / 9  &  -0.16 / 11  &  -0.11 / 5  & -0.14 / 8 \\
PropOpposition  &  -0.24 / 9  &  -0.04 / 9  &  -0.14 / 10  &  -0.23 / 8  &  -0.05 / 9  & -0.14 / 9 \\
    \hline
    \end{tabular}
\end{center}
\caption{Correlation (correlation score / feature rank) of \textit{Expert} features to the real and predicted mean-ages at the text and sentence levels}
\label{table:correlation} 
\vspace{-4mm}
\end{table}

%First correlation is measured between each expert-feature and the real ages at the sentence and text levels, and then done similar with the recommended ages for two models, [GRU/T\textsubscript{CB}, Feed-forward/GRU\_pred.$\oplus$T\textsubscript{Expert}] (for text level recommendation) and [CamemBERT/-, Feed-forward/CamemBERT\_pred.$\oplus$S\textsubscript{Expert}] (for sentence level recommendation). 
First correlation is measured between each expert-feature and the real ages at the sentence and text levels, and then done similar with the predicted ages from two models, GRU/T\textsubscript{CB} (text level) and CamemBERT/- (sentence level) as shown in Fig.~\ref{fig:correlation}. 
We hypothesize that the top ranked correlated features will be similar for the real age and recommended age for a good age recommendation model. 
%This section refers Pearson correlation coefficient as the correlation score.
Table~\ref{table:correlation} shows the top 10 positively correlated (upper part) and top 10 negatively correlated (bottom part) features with different settings. Each correlation score is presented with its rank among the features. For example, in second column (Real Age/Text), the correlation score for \textit{PhonemeNumberStd} (0.58 / 1) is 0.58 with the rank of 1. From this table, it is very clear that the top 10 positively correlated features are common in all settings although their ranks displace a little. Similar characteristics is observed for the top 10 negatively correlated features as well. 
%From the correlation based feature ranking, one can notice that the most important features include \textit{Phonetics}, \textit{SentenceLength} and \textit{DependencyMaxDistance}. 
From the correlation based feature ranking, one can notice that among different types of features the \textit{phonetic} features obtains the best rank scores.

\subsection{Permutation Feature Ranking}
The idea of permutation feature ranking is to randomly shuffle an individual feature value to break the relationship between the feature and the target value. Thus it measures the drop of performance due to discarding the feature, and finally ranks the features. Here we do it for the expert features (T\textsubscript{Expert} and S\textsubscript{Expert}) at the sentence level and text level on the test set by employing Random Forest regressor, a built-in library in scikit-learn. 
%First, feature ranking is performed with the expert features (T\textsubscript{Expert} and S\textsubscript{Expert}) at the sentence and text levels, and then combining them with the GRU\_pred. ages (text level) and CamemBERT\_pred. ages (sentence level) as additional features.

\begin{table}[t]
    % \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l|}
      \hline
      \multicolumn{2}{|c|}{\textbf{Sentence Level}} & \multicolumn{2}{c|}{\textbf{Text Level}}\\
      \hline
% 	  \textbf{Sentence level} & \textbf{Text level} \\ \hline
    \textbf{Feature} & \textbf{Score} & \textbf{Feature} & \textbf{Score} \\ \hline

PhonemeNumberAvg & 0.1021 & PhonemeNumberAvg & 0.1596 \\
PhonemeNumberStd & 0.0383 & SentenceLength & 0.1425 \\
SentenceLength & 0.0368 & PhonemeNumberStd & 0.0847 \\
PhonemeProbStd & 0.0132 & PhonemeProbStd & 0.0245 \\
StopWordsProportion & 0.0130 & PolarityScore & 0.0213 \\
NumberOfDependenciesAvg & 0.0110 & PhonemeProbSentence & 0.0180 \\
DependencyMaxDistance & 0.0086 & DependencyMaxDistance & 0.0164 \\
WordProbAvg & 0.0076 & StopWordsProportion & 0.0151 \\
PhonemesDiversityAvg & 0.0069 & WordProbAvg & 0.0143 \\
PhonemesDiversityStd & 0.0063 & GraphemeConfusionAvg & 0.0142 \\
     \hline
    \end{tabular}
\end{center}
\caption{Top 10 \textit{Expert} features (with rank-scores) by permutation feature ranking at the sentence and text levels}
\label{table:permutation feature ranks} 
\vspace{-4mm}
\end{table}

Table~\ref{table:permutation feature ranks} enlists the top 10 features for different feature combinations at the sentence and text levels. For ranking on the \textit{Expert} features, most of the top ranked features are related to \textit{Phonetics}. Moreover, the \textit{SentenceLength}, \textit{DependencyMaxDistance} and \textit{StopWordsProportion} are found very important features for age recommendation at the sentence and text levels. These features are also seen in the list of top 10 features by correlation based feature ranking in Table~\ref{table:correlation}.

% However, when the ranking is done by Expert$\oplus$[CamemBERT\_pred. or GRU pred.] features, CamemBERT or GRU recommended ages are ranked as the most contributory features at sentence and text levels. Interestingly, the rest of the important features differ significantly between the sentence and text levels. Moreover, for Expert$\oplus$[CamemBERT\_pred. or GRU pred.] setting, the top-ranked \textit{Expert} features do not include the \textit{Phonetics}, \textit{SentenceLength} and \textit{DependencyMaxDistance} features. The reason may be that CamemBERT has already considered these information in its training phase.


\subsection{Ablation Test}
Finally we do an ablation test with different categories of the \textit{Expert} features on the test set. The idea of ablation test is like the permutation feature ranking where an individual feature is shuffled and its impact on the performance is measured. Here ablation test is done with the Feed-forward model,
but instead of shuffling a single feature, all the features of same category are discarded.

% \begin{table}[t]
%     %\small
% \begin{center}
% 	\setlength{\tabcolsep}{2pt}
% 	\renewcommand{\arraystretch}{1.3}
% 	\begin{tabular}{|l|l|l||l|l|}
% 	 \hline
%      & \multicolumn{2}{c|}{\textbf{Sentence Level}} & \multicolumn{2}{c|}{\textbf{End-to-end Text Level}}\\
%       \hline
% 	  \textbf{Features} & \textbf{MAE} & \textbf{MBE} & \textbf{MAE} & \textbf{MBE} \\ \hline
% Expert & 2.68 & 1.42 & 2.13 & 0.84 \\ \hdashline
% Expert-Dependencies & 2.71 & 1.44 & 2.27 & 0.94 \\
% Expert-Person/Number & 2.68 & 1.42 & 2.16 & 0.86 \\
% Expert-Graphemes & 2.65 & 1.39 & 2.18 & 0.87 \\
% Expert-Lexicon & 2.69 & 1.42 & 2.29 & 0.95 \\
% Expert-VerbalTenses& 2.66 & 1.40 & 2.19 & 0.88 \\
% Expert-Phonetics & 2.77 & 1.49 & 2.33 & 0.97 \\
% Expert-Morphosyntax & 2.71 & 1.45 & 2.26 & 0.94 \\
% Expert-Connectors& 2.67 & 1.42 & 2.21 & 0.93 \\
% Expert-Sentiments & 2.69 & 1.43 & 2.18 & 0.85 \\ \hline
%     \end{tabular}
% \end{center}
% \caption{Ablation test MAE (mean-age) and MBE}
% \label{table:Ablation test MAE and MBE} 
% \end{table}


\begin{table}[t]
    %\small
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|}
	 \hline
	  \textbf{Features} & \textbf{Sentence} & \textbf{Text} \\ \hline
\textbf{Expert} & \textbf{2.66} & \textbf{2.22} \\ \hline
Expert - Phonetics & 2.77 / +0.11 & 2.33 / +0.11 \\
Expert - Dependencies & 2.71 / +0.05 & 2.27 / +0.05 \\
Expert - Morphosyntax & 2.71 / +0.05 & 2.26 / +0.04 \\
Expert - Lexicon & 2.69 / +0.03 & 2.29 / +0.07 \\
\hdashline
\hdashline
Expert - Sentiments & 2.69 / +0.03 & 2.18 / -0.04 \\
Expert - Person/Number & 2.68 / +0.02 & 2.16 / -0.06 \\
Expert - Connectors & 2.67 / +0.01 & 2.21 / -0.01 \\
Expert - VerbalTenses & 2.66 / +0.00 & 2.19 / -0.03 \\
Expert - Graphemes & 2.65 / -0.01 & 2.18 / -0.04 \\
\hline
    \end{tabular}
\end{center}
\caption{Ablation test ($\mu{}E$ / $\Delta$) of the \textit{Expert} features with Feed-forward model at the sentence and text levels}
\label{table:Ablation test muE} 
\vspace{-4mm}
\end{table}

Table~\ref{table:Ablation test muE} presents the $\mu{}E$ scores of the ablation test where almost all the feature categories except \textit{VerbalTenses} and \textit{Graphemes} show positive impacts at sentence level. Interestingly, the \textit{Phonetics, Dependencies, Morphosyntax} and \textit{Lexicon} features have positive impacts at both sentence and text levels. All the feature ranking approaches studied in this paper find the phonetics and dependency features the most common and contributory in any settings. Although these feature categories individually do not have very high impact, they altogether perform quite well in age recommendation task.

==> section_7_feature_analysis_FR.tex <==
\section{Feature Analysis}
\label{sec:feature_analysis}
% data stat: 
% about the features
% scores per age

Overall the age prediction models obtain very decent scores. Although the expert-feature set along does not achieve the best score, it allows us to analyse which linguistic properties have higher contributions for age prediction. This section explores feature selection by different approaches.

\subsection{Correlation Between Feature and Age}
At this point, we are interested to measure the correlation between the features and age (on test set) to identify the most contributory features. First correlation is measured between each expert-feature and the real ages at the sentence and text levels, and then done similar with the predicted ages for two models, GRU/CamemBERT and Expert+GRU/CamemBERT Pred. We hypothesize that the top ranked correlated features will be similar for the real age and predicted age for a good age prediction model. This section refers Pearson correlation coefficient as the correlation score.

\begin{table}[t]
    \scriptsize
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|l||l|l|l|l|l|}
	 \hline
     & \multicolumn{3}{c||}{\textbf{Real Age}} & \multicolumn{5}{c|}{\textbf{Predicted Age}}\\
      \hline
      & \multicolumn{3}{c||}{} & \multicolumn{2}{c|}{\textbf{GRU/CamemBERT}} & \multicolumn{2}{c|}{\textbf{Expert+GRU/CamemBERT}} & \\
      \hline
	  \textbf{Features} & \textbf{Text} & \textbf{Sent.} & \textbf{Avg.*} & \textbf{Text} & \textbf{Sent.} & \textbf{Text} & \textbf{Sent.} & \textbf{Avg.} \\ \hline
nbPhonemeMoyen & 0.56 / 2 & 0.25 / 1 & 0.40 / 1 & 0.48 / 3 & 0.27 / 1 & 0.53 / 3 & 0.23 / 1 & 0.38 / 2 \\
nbPhonemeVariance & 0.58 / 1 & 0.22 / 2 & 0.40 / 2 & 0.52 / 1 & 0.26 / 2 & 0.56 / 1 & 0.20 / 5 & 0.38 / 1 \\
VarianceLongueurMots & 0.54 / 3 & 0.19 / 7 & 0.37 / 3 & 0.50 / 2 & 0.25 / 4 & 0.53 / 2 & 0.20 / 8 & 0.37 / 3 \\
DiversitéLemmes & 0.50 / 4 & 0.22 / 4 & 0.36 / 4 & 0.48 / 6 & 0.24 / 5 & 0.49 / 5 & 0.21 / 3 & 0.35 / 5 \\
longueur\_phrase & 0.49 / 5 & 0.22 / 3 & 0.36 / 5 & 0.48 / 4 & 0.25 / 3 & 0.49 / 6 & 0.21 / 2 & 0.36 / 4 \\
LongueurMotsMoyenne & 0.49 / 6 & 0.20 / 5 & 0.35 / 6 & 0.43 / 8 & 0.23 / 6 & 0.47 / 7 & 0.20 / 6 & 0.33 / 7 \\
ProportionSymboles & 0.49 / 7 & 0.20 / 6 & 0.35 / 7 & 0.43 / 9 & 0.23 / 7 & 0.47 / 8 & 0.20 / 7 & 0.33 / 8 \\
ProfArbDep & 0.48 / 8 & 0.19 / 8 & 0.34 / 8 & 0.48 / 5 & 0.22 / 8 & 0.50 / 4 & 0.20 / 4 & 0.35 / 6 \\
depDistMax & 0.47 / 9 & 0.18 / 9 & 0.32 / 9 & 0.44 / 7 & 0.20 / 9 & 0.46 / 9 & 0.18 / 9 & 0.32 / 9 \\
VarianceConfusion & 0.47 / 10 & 0.16 / 10 & 0.31 / 10 & 0.41 / 10 & 0.20 / 10 & 0.45 / 10 & 0.16 / 10 & 0.30 / 10 \\
% ConfusionMoyenne & 0.40 / 11 & 0.15 / 11 & 0.27 / 11 & 0.32 / 14 & 0.17 / 11 & 0.35 / 13 & 0.14 / 11 & 0.25 / 11 \\
% PointDistMoy & 0.39 / 12 & 0.12 / 12 & 0.26 / 12 & 0.34 / 12 & 0.13 / 13 & 0.38 / 11 & 0.13 / 12 & 0.24 / 13 \\
% PointDistVar & 0.38 / 13 & 0.10 / 14 & 0.24 / 13 & 0.37 / 11 & 0.13 / 12 & 0.37 / 12 & 0.11 / 13 & 0.25 / 12 \\
% depDistMoy & 0.36 / 14 & 0.12 / 13 & 0.24 / 14 & 0.33 / 13 & 0.12 / 14 & 0.35 / 14 & 0.11 / 14 & 0.23 / 14 \\
% NombreMoyenDedependances & 0.28 / 15 & 0.09 / 15 & 0.19 / 15 & 0.23 / 15 & 0.07 / 17 & 0.26 / 15 & 0.10 / 16 & 0.17 / 15 \\
\hline
\hline
nbPhonemePhrase & -0.34 / 2 & -0.15 / 1 & -0.25 / 1 & -0.31 / 3 & -0.16 / 1 & -0.34 / 3 & -0.14 / 1 & -0.24 / 2 \\
DiversitéPhonemesPhrase & -0.34 / 3 & -0.15 / 2 & -0.25 / 2 & -0.31 / 4 & -0.16 / 2 & -0.34 / 4 & -0.14 / 2 & -0.24 / 3 \\
FrequencePhonemesVariance & -0.37 / 1 & -0.10 / 4 & -0.24 / 3 & -0.39 / 1 & -0.15 / 3 & -0.43 / 1 & -0.12 / 4 & -0.27 / 1 \\
DiversitéPhonemesVariance & -0.32 / 6 & -0.14 / 3 & -0.23 / 4 & -0.25 / 6 & -0.15 / 4 & -0.30 / 6 & -0.14 / 3 & -0.21 / 4 \\
ProportionStopWords & -0.33 / 5 & -0.08 / 5 & -0.20 / 5 & -0.31 / 5 & -0.09 / 6 & -0.32 / 5 & -0.05 / 6 & -0.19 / 5 \\
PropTemps & -0.34 / 4 & -0.04 / 10 & -0.19 / 6 & -0.32 / 2 & -0.04 / 10 & -0.35 / 2 & -0.04 / 9 & -0.19 / 6 \\
amour & -0.29 / 8 & -0.06 / 7 & -0.17 / 7 & -0.23 / 7 & -0.07 / 7 & -0.27 / 7 & -0.05 / 7 & -0.15 / 7 \\
joie & -0.29 / 7 & -0.05 / 8 & -0.17 / 8 & -0.17 / 10 & -0.06 / 8 & -0.22 / 9 & -0.04 / 8 & -0.12 / 10 \\
VarianceFrequence & -0.21 / 10 & -0.08 / 6 & -0.14 / 9 & -0.16 / 11 & -0.11 / 5 & -0.22 / 10 & -0.10 / 5 & -0.14 / 8 \\
PropOpposition & -0.24 / 9 & -0.04 / 9 & -0.14 / 10 & -0.23 / 8 & -0.05 / 9 & -0.23 / 8 & -0.04 / 10 & -0.14 / 9 \\
% comportement & -0.18 / 11 & -0.03 / 12 & -0.10 / 11 & -0.19 / 9 & -0.04 / 11 & -0.20 / 11 & -0.03 / 12 & -0.11 / 11 \\
% peur & -0.16 / 12 & -0.04 / 11 & -0.10 / 12 & -0.14 / 12 & -0.02 / 13 & -0.16 / 12 & -0.02 / 13 & -0.09 / 12 \\
% ProportionAdvTemp & -0.12 / 13 & -0.02 / 14 & -0.07 / 13 & 0.00 / 25 & -0.02 / 14 & -0.13 / 13 & -0.03 / 11 & -0.05 / 16 \\
% PropAddition & -0.11 / 14 & -0.02 / 17 & -0.06 / 14 & 0.01 / 26 & -0.02 / 16 & -0.10 / 16 & -0.01 / 20 & -0.03 / 18 \\
% PropEnumeration & -0.08 / 16 & -0.02 / 13 & -0.05 / 15 & 0.11 / 24 & -0.01 / 22 & -0.07 / 18 & -0.01 / 19 & 0.00 / 28 \\
    \hline
    \end{tabular}
\end{center}
\caption{Correlation (correlation score / feature rank) of Expert-features to the real and predicted mean-ages at the text and sentence levels}
\label{table:correlation} 
\end{table}

Table~\ref{table:correlation} shows the top 10 positively correlated (upper part) and top 10 negatively correlated (bottom part) features with different settings. Each correlation score is presented with its rank among the features. For example, in second column (Real Age/Text), the correlation score for \textit{nbPhonemeVariance} (0.58 / 1) is 0.58 with the rank of 1. From this table, it is very clear that the top 10 positively correlated features are common in all settings although their ranks displace a little. Similar characteristics is observed for the top 10 negatively correlated features as well. From the correlation based feature ranking, one can notice that the most important features include \textit{phonetics}, \textit{sentence\_length} and \textit{depDistMax}. These features are also listed in the top 10 of permutation feature ranking with expert-features in Table~\ref{table:permutation feature ranks}.

\subsection{Permutation Feature Ranking}
The idea of permutation feature ranking is to randomly shuffle an individual feature value to break the relationship between the feature and the target value. Thus it measures the drop of performance due to discarding the feature, and finally ranks the features. Here we do it on the test set by employing Random Forest regressor, a built-in library in scikit-learn. First, feature ranking is performed with the expert features at the sentence and text levels, and then combining them with the CamemBERT/GRU predicted ages as features.

\begin{table}[t]
    \tiny
\begin{center}
	\setlength{\tabcolsep}{2pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l||l|l|}
	 \hline
     \multicolumn{2}{|c||}{\textbf{Expert}} & \multicolumn{2}{c|}{\textbf{Expert+CamemBERT/GRU pred.}}\\
      \hline
	  \textbf{Sentence level} & \textbf{Text level} & \textbf{Sentence level} & \textbf{Text level} \\ \hline
% 	  nbPhonemeMoyen & nbPhonemeMoyen & CamemBertPredMaxAge & GruPredMinAge \\
% nbPhonemeVariance & longueur\_phrase & CamemBertPredMinAge & GruPredMaxAge \\
% longueur\_phrase & nbPhonemeVariance & tristesse & FréquencePhonèmesPhrase \\
% FrequencePhonemesVariance & FrequencePhonemesVariance & surprise & MoyFreqOccurence \\
% ProportionStopWords & score\_de\_polarite & PropEnumeration & LongueurMotsMoyenne \\
% NombreMoyenDedependances & FréquencePhonèmesPhrase & comportement & FrequenceMoyenne \\
% depDistMax & depDistMax & mepris & NombreMoyenDedependances \\
% MoyFreqOccurence & ProportionStopWords & PropConclusion & neutre \\
% DiversitéPhonemesMoyenne & MoyFreqOccurence & ProportionAdvTemp & ProportionSymboles \\
% DiversitéPhonemesVariance & ConfusionMoyenne & orgueil & ProfArbDep \\


nbPhonemeMoyen (0.1021) & nbPhonemeMoyen (0.1596) & CamemBertPredMaxAge (0.2400) & GruPredMinAge (0.4634) \\
nbPhonemeVariance (0.0383) & longueur\_phrase (0.1425) & CamemBertPredMinAge (0.2099) & GruPredMaxAge (0.4017) \\
longueur\_phrase (0.0368) & nbPhonemeVariance (0.0847) & tristesse (0.0003) & FréquencePhonèmesPhrase (0.0041) \\
FrequencePhonemesVariance (0.0132) & FrequencePhonemesVariance (0.0245) & surprise (0.0002) & MoyFreqOccurence (0.0030) \\
ProportionStopWords (0.0130) & score\_de\_polarite (0.0213) & PropEnumeration (0.0002) & LongueurMotsMoyenne (0.0024) \\
NombreMoyenDedependances (0.0110) & FréquencePhonèmesPhrase (0.0180) & comportement (0.0001) & FrequenceMoyenne (0.0023) \\
depDistMax (0.0086) & depDistMax (0.0164) & mepris (0.0001) & NombreMoyenDedependances (0.0019) \\
MoyFreqOccurence (0.0076) & ProportionStopWords (0.0151) & PropConclusion (0.0001) & neutre (0.0013) \\
DiversitéPhonemesMoyenne (0.0069) & MoyFreqOccurence (0.0143) & ProportionAdvTemp (0.0001) & ProportionSymboles (0.0010) \\
DiversitéPhonemesVariance (0.0063) & ConfusionMoyenne (0.0142) & orgueil (0.0001) & ProfArbDep (0.0008) \\

% VarFreqOccurence & FrequenceMoyenne & PropTemps & PropCause \\
% DiversitéPhonemesPhrase & DiversitéLemmes & empathie & FrequencePhonemesMoyenne \\
% nbPhonemePhrase & VarianceConfusion & fierte & DiversitéPhonemesMoyenne \\
% FrequenceMoyenne & ProfArbDep & PropCause & VarFreqOccurence \\
% FréquencePhonèmesPhrase & PropConsequence & apaisement & depDistMoy \\
      \hline
    \end{tabular}
\end{center}
\caption{Top 10 Expert-features (with rank-scores) by permutation feature ranking at the sentence and text levels}
\label{table:permutation feature ranks} 
\end{table}

Table~\ref{table:permutation feature ranks} enlists the top 10 features for different feature combinations at the sentence and text levels. For ranking on the expert-features, most of the top ranked features are related to \textit{phonetics}. Moreover, the \textit{sentence\_length}, \textit{depDistMax} and \textit{proportionStopWords} are found very important features for age prediction at the sentence and text levels. However, when the ranking is done by Expert+CamemBERT/GRU pred. features, CamemBERT/GRU predicted ages are ranked as the contributory features for sentence and text levels. Interestingly, the rest of the important features differ significantly between the sentence and text levels. Moreover, for Expert+CamemBERT/GRU pred. setting, the top-ranked expert features do not include the \textit{phonetics}, \textit{sentence\_length} and \textit{depDistMax} features. The reason may be that CamemBERT has already considered these information.


\subsection{Ablation Test}
Finally we do ablation test with different categories of the expert-features on the test set. The idea of ablation test is like the permutation feature ranking where an individual feature is shuffled and its impact on the performance is measured. Here ablation test is done with the Feed-forward model,
but instead of shuffling a single feature, all the features of same category are discarded.

% \begin{table}[t]
%     %\small
% \begin{center}
% 	\setlength{\tabcolsep}{2pt}
% 	\renewcommand{\arraystretch}{1.3}
% 	\begin{tabular}{|l|l|l||l|l|}
% 	 \hline
%      & \multicolumn{2}{c|}{\textbf{Sentence Level}} & \multicolumn{2}{c|}{\textbf{End-to-end Text Level}}\\
%       \hline
% 	  \textbf{Features} & \textbf{MAE} & \textbf{MBE} & \textbf{MAE} & \textbf{MBE} \\ \hline
% Expert & 2.68 & 1.42 & 2.13 & 0.84 \\ \hdashline
% Expert-Dependances & 2.71 & 1.44 & 2.27 & 0.94 \\
% Expert-PersonnesNombres & 2.68 & 1.42 & 2.16 & 0.86 \\
% Expert-Graphie & 2.65 & 1.39 & 2.18 & 0.87 \\
% Expert-Lexique & 2.69 & 1.42 & 2.29 & 0.95 \\
% Expert-Temps\_Verbaux & 2.66 & 1.40 & 2.19 & 0.88 \\
% Expert-Phonetique & 2.77 & 1.49 & 2.33 & 0.97 \\
% Expert-Morphosyntaxe & 2.71 & 1.45 & 2.26 & 0.94 \\
% Expert-Connecteurs & 2.67 & 1.42 & 2.21 & 0.93 \\
% Expert-Sentiments & 2.69 & 1.43 & 2.18 & 0.85 \\ \hline
%     \end{tabular}
% \end{center}
% \caption{Ablation test MAE (mean-age) and MBE}
% \label{table:Ablation test MAE and MBE} 
% \end{table}


\begin{table}[t]
    %\small
\begin{center}
	\setlength{\tabcolsep}{4pt}
	\renewcommand{\arraystretch}{1.3}
	\begin{tabular}{|l|l|l|}
	 \hline
	  \textbf{Features} & \textbf{Sentence} & \textbf{Text} \\ \hline
\textbf{Expert} & \textbf{2.66} & \textbf{2.22} \\ \hline
Expert - Phonetique & 2.77 / +0.11 & 2.33 / +0.11 \\
Expert - Dependances & 2.71 / +0.05 & 2.27 / +0.05 \\
Expert - Morphosyntaxe & 2.71 / +0.05 & 2.26 / +0.04 \\
Expert - Lexique & 2.69 / +0.03 & 2.29 / +0.07 \\
\hdashline
Expert - Sentiments & 2.69 / +0.03 & 2.18 / -0.04 \\
Expert - PersonnesNombres & 2.68 / +0.02 & 2.16 / -0.06 \\
Expert - Connecteurs & 2.67 / +0.01 & 2.21 / -0.01 \\
Expert - Temps\_Verbaux & 2.66 / +0.00 & 2.19 / -0.03 \\
Expert - Graphie & 2.65 / -0.01 & 2.18 / -0.04 \\
\hline
    \end{tabular}
\end{center}
\caption{Ablation test ($\mu{}E$ / $\Delta$) of the Expert-features with Feed-forward model at the sentence and text levels}
\label{table:Ablation test muE} 
\end{table}

Table~\ref{table:Ablation test muE} presents the $\mu{}E$ scores of the ablation test where almost all the feature categories except \textit{verbal\_tenses} and \textit{grapheme} show positive impacts at sentence level. Interestingly, the \textit{phonetics, dependency, morpho-syntactic} and \textit{lexical} features have positive impacts at both sentence and text levels. All the feature ranking approaches studied in this paper find the phonetics and dependency features the most common and contributory in any settings. Although these feature categories individually do not have very high impact, they altogether perform quite well in age prediction task.
